From Multisets to Sets in Hotmotopy Type Theory

We give a model of set theory based on multisets in homotopy type theory. The equality of the model is the identity type. The underlying type of iterative sets can be formulated in Martin-L\"of type theory, without Higher Inductive Types (HITs), and is a sub-type of the underlying type of Aczel's 1978 model of set theory in type theory. The Voevodsky Univalence Axiom and mere set quotients (a mild kind of HITs) are used to prove the axioms of constructive set theory for the model. We give an equivalence to the model provided in Chapter 10 of "Homotopy Type Theory" by the Univalent Foundations Program.

==> iterative-sets/collection.tex <==
\section{Collection axioms}\label{collection-axioms}

In this section we discuss the status of collection axioms of
constructive set theory in our model.

Neither strong collection, nor subset collection seem to hold in either
extreme interpretation of the existential quantifier (i.e.~applying τ or
σ). Interpreting the existential quantifier as \(Σ\)-types forces us to
make arbitrary choices in an apparently unconstructive way. Interpreting
the existential quantifier as the truncated ∃, the assumptions become
too weak to work with.

We discuss two approaches to solving this problem. On the one hand, we
identify which existential quantifiers need to be weakened -- and which
have to remain strict -- in order to get something like the collection
axioms to become provable for our model. On the other hand, we identify
axioms about the type theoretical universe, from which \(V\) was
constructed, from which we can derive collection and subset collection
in the truncated form.

\subsection{Strong Collection}\label{strong-collection}

Together with subset collection, strong collection is the most subtle of
the axioms of constructive set theory. First of all because it is
underspecified: the strong collection axiom states the existence of a
set, but does not define it up to equality.

On an intuitive level, strong collection states that if we have shown
that for all elements of a set \(x\) there exists some element with a
certain property, then the proof is in some way an operation which
should have an image in \(V\).

The problem is that the proof in first-order logic may not be uniform,
in the sense that the operation may not respect equality of elements.
However, this would not prevent us from taking its image.

In Aczel's original model one can see this, as his \(V\) is a setoid and
we can talk about extensional operations on the underlying type.
However, our \(V\) has the identity type as its equality type. This
means that if we interpret the existential quantifier as the Σ-type,
then any proof operation will give rise to an actual function which
respects equality. The image of such an operation is naturally a
multiset, and we have seen how to quotient such a multiset to a set. The
only wrinkle of this approach is that the ``strong part'' of strong
collection has to be weakened by using a truncated existential
quantifier.

\subsubsection{Strong quantifiers}\label{strong-quantifiers}

The following proposition is the rendering of strong collection in which
we, as far as our abilities go, interpreted the existential quantifier
as Σ-types.

\paragraph{Proposition}\label{proposition}

\label{collection-balenced}

For any predicate \(P : V → V → \Type\) and every \(a : V\) if
\(∏_{x : V} (x ∈ a) → ∑_{y : V} P␣x␣y\) then there is \(b : V\) such
that

\begin{enumerate}
\itemsep1pt\parskip0pt\parsep0pt
\item
  \(∏_{x:V} (x ∈ a) → ∑_{y : V} y ∈ b ∧ (P␣x␣y)\)
\item
  \(∏_{y:V} (y ∈ b) → ∃(x : V)\ x ∈ a ∧ (P␣x␣y)\)
\end{enumerate}

\emph{Proof:} Given \(a ≡ \sup␣\bar a␣\tilde a\), the assumptions let us
construct a map \(T␣\bar a → V\). Using Lemma \ref{image-lemma}, we can
construct its image in \(V\), which will have the desired properties.∎

\paragraph{Remark}\label{remark}

It is well known that, in constructive set theory, collection implies
replacement, and that the converse implication does not hold. But the
strong version of replacement proven for our model in Proposition
\ref{replacement}, formulated for a given ∈-structure, does in fact
entail the collection principle of Proposition
\ref{collection-balenced}, for the same ∈-structure.

\subsubsection{Weak quantifies}\label{weak-quantifies}

\textcite{gambino2006} discuss a general approach to interpreting
first-order logic into type theory. For any given interpretation in
their framework, they identify type theoretic principles corresponding
to strong collection and subset collection. Here we will, in a similar
fashion, give a sufficient principle for our model to satisfy strong
collection in the sense of weak quantifiers.

\paragraph{Definition}\label{definition}

\textbf{Collection Principle for a universe, \(U\):}

For every locally \(U\)-small \(B : \Set\), given \(a : U\) and
\(P : T␣a → B → \Type\), such that \(∏_{x:T␣A} ∃(y : B)P␣x␣y\) then
\(∃(r : U) ∃(β : T␣r ↪ B) (∏_{x:T␣a}∃(y:T␣r)P␣x␣(β␣y))∧(∏_{y : T␣r}∃(x : T␣a)P␣x␣y)\).

\paragraph{Proposition}\label{proposition-1}

The collection principle for \(U\) implies strong collection in the
following sense:

For any predicate \(P : V → V → \Type\) and every \(a : V\) if
\(∏_{x : V} (x ∈ a) → ∃(y : V) P␣x␣y\) then there merely exists
\(b : V\) such that

\begin{enumerate}
\itemsep1pt\parskip0pt\parsep0pt
\item
  \(∏_{x:V} (x ∈ a) → ∃(y : V)\ y ∈ b ∧ (P␣x␣y)\)
\item
  \(∏_{y:V} (y ∈ b) → ∃(x : V)\ x ∈ a ∧ (P␣x␣y)\)
\end{enumerate}

\emph{Proof:} Apply the collection principle for \(U\) to
\(P ∘ \bar a\), to obtain the mere existence \(r\) and \(β\), which
together form \(b≔\sup␣r␣β\). 1. and 2. follow from the property of the
collection principle for \(U\). ∎

\subsection{Subset Collection}\label{subset-collection}

Subset collection is the principle that for any pair of sets there is a
third set, such that each total relation between the two has an image in
the third. The precise formulation of the axiom in first-order logic is
slightly complicated by the fact that one cannot quantify over all (or
even all definable) total relations in the middle of a formula.
Therefore, the axiom is an axiom schema quantified over ternary
formulas, where the first parameter is allowed to vary. Our formulation
will be close to the first-order formulation:

\begin{align*}
∀ a,b\ ∃c\ ∀ u\ (∀ x∈ a& → ∃y ∈ b ∧ P␣u␣x␣y)\\
→ (∃d∈c &∧ (∀x∈ a → ∃y ∈ d ∧ P␣u␣x␣y) \\
           &∧ (∀y∈d → ∃x\ x ∈ a ∧ P␣u␣x␣y)
\end{align*}

In the above formula there are three existential quantifiers to
interpret, either as a Σ-type or as a truncated existential. At one
extreme it is possible to give all but the last existential quantifier
the Σ-type interpretation, truncating the last one.

\paragraph{Proposition}\label{proposition-2}

For every predicate \(P : V → V → V → \Type\) and every \(a,b : V\)
there is \(c : V\) such that for all \(u : V\) if
\(∏_{x : V} (x ∈ a) → ∑_{y : V} P␣u␣x␣y\) then there is \(d ∈ c\) such
that

\begin{enumerate}
\itemsep1pt\parskip0pt\parsep0pt
\item
  \(∏_{x:V} (x ∈ a) → ∑_{y : V} y ∈ d ∧ (P␣u␣x␣y)\)
\item
  \(∏_{y:V} (y ∈ d) → ∃(x : V)\ x ∈ a ∧ (P␣u␣x␣y)\)
\end{enumerate}

\emph{Proof:} Given \(a ≡ \sup␣\bar a␣\tilde a\) and
\(b ≡ \sup␣\bar b␣\tilde b\), consider the function
\(γ:(\bar a → \bar b) → V\) which maps each \(f : \bar a → \bar b\) to
\(\image (\tilde b ∘ f)\) in \(V\). Let \(c ≔ \image␣γ\), which will
have the desired properties.∎

\subsubsection{Weak quantifiers}\label{weak-quantifiers}

In the same way we did for strong collection, we identify a principle of
subset collection for our universe which is sufficient to prove the
truncated variation of subset collection for our model.

\paragraph{Definition}\label{definition-1}

\textbf{Subset Collection Principle for \(U\):}

For each \(a,b:U\) there merely exists \(c:U\) such that for every
\(P:T␣a→T␣b→\Type\) such that \(∏_{x:T␣a}∃(y:T␣b)P␣x␣y\), there
\(∃(r : T␣c) (∏_{x:T␣a}∃(y:T␣r)P␣x␣(α␣y)) ∧ (∏_{y : T␣r}∃(x : T␣a)P␣x␣y)\)

\paragraph{Proposition}\label{proposition-3}

For every predicate \(P : V → V → V → \Type\) and every \(a,b : V\),
there merely exists a \(c : V\) such that for every \(u : V\), if
\(∏_{x : V} (x ∈ a) → ∑_{y : V} P␣u␣x␣y\) then there merely exists
\(d ∈ c\) such that

\begin{enumerate}
\itemsep1pt\parskip0pt\parsep0pt
\item
  \(∏_{x:V} (x ∈ a) → ∃(y : V)\ y ∈ d ∧ (P␣u␣x␣y)\)
\item
  \(∏_{y:V} (y ∈ d) → ∃(x : V)\ x ∈ a ∧ (P␣u␣x␣y)\)
\end{enumerate}

\emph{Proof:} Apply the subset collection principle for \(U\) to
\(a\),\(b\) to obtain the mere existence of \(c\), and then use the
property of \(c\) on the predicate \(P␣u\).


==> iterative-sets/hit.tex <==
\section{Equivalence with the
HIT-formulation}\label{equivalence-with-the-hit-formulation}

Section 5.1 of Chapter 10 of the book ``Homotopy Type Theory''
\footcite{hottbook}, is dedicated to set theory in the context of
homotopy type theory. The iterative hierarchy is presented there, in the
form of a higher inductive type (HIT). Our \(V\) is a HIT-free
alternative to this, and in this section we show that the two types are
equivalent.

The HIT formulation bears more than a slight similarity to Aczel's
original construction of the iterative hierarchy in type theory. Both
are quotients of the type we call \(M\). The difference is that while
Aczel uses the untruncated version of the quantifiers and leaves the
quotient a setoid, HTT uses the truncated quantifiers and postulates the
existence of a type with the identity type to match.

In this section we define the bisimulation relation on \(M\) of which
the \(V\) in HTT Chapter 10 can be seen a quotient. We show that this
quotient is equivalent to our \(V\). The proof on this relies on a
function, \(\itimage : M → V\), which turns any multiset into an
iterative set by identifying all occurrences of each elements, having
first applied the process inductively on all elements.

\paragraph{Definition}\label{definition}

We define by induction on \(M\) the binary relation:

\begin{align*}
≈ &: M → M → \Type \\
(\sup␣a␣f) ≈ (\sup␣b␣g)
   &≔ \left(∏_{x:T␣a} ∃ (y:T␣b) ({f␣x} ≈ {g␣y})\right) \\
   &× \left(∏_{y:T␣b} ∃ (x:T␣a) ({f␣x} ≈ {g␣y})\right)
\end{align*}\vspace{3mm}

\paragraph{Definition}\label{definition-1}

We define by induction on \(M\) the function:

\begin{align*}
 &\itimage : M → V \\
 &\itimage␣(\sup␣a␣f) ≔ \image␣a␣(\itimage ∘ f)
\end{align*}

\paragraph{Lemma}\label{lemma}

For each \(x : M\) we have that \(x ≈ \itimage␣x\).

\emph{Proof:} For each element of \(x\) there is a corresponding element
in \(\itimage␣x\), since the type of elements of \(\itimage␣x\) is a
quotient of the type of elements in \(x\). In the other direction there
just \emph{merely} exists an element of \(x\) for each element of
\(\itimage␣x\), since it was a quotient. However, this is sufficient to
show that \(x ≈ \itimage␣x\).

\paragraph{Lemma}\label{lemma-1}

For iterative sets \(≈\) is equivalent to the identity type. That is,
for every \(x,y : M\) given \(\itset␣x\) and \(\itset␣y\), we have that
\(x ≈ y → x =_M y\).

\emph{Proof:} By W-induction. Let \(x≡\sup␣a␣f\) and \(y≡\sup␣b␣g\), and
assume \(x ≈ y\). By extensionality, it suffices to show that for any
\(z : M\) we have that \(z ∈_M x\) if and only if \(z ∈_M y\).

In one direction, if \(z ∈_M x\) we know that there is \(i : T␣a\) such
that \(z =_M f␣i\). Since \(z ∈_M y\) is a mere proposition, we can
assume from \(x ≈ y\) that there is a \(j : T␣b\) such that
\({f␣i} ≈ {g␣j}\). By inductive hypothesis,
\({f␣i} ≈ {g␣j} → f␣i =_M g␣j\), and thus \(z =_M g␣j\) which is to say
\(z ∈_M y\).

The other direction is symmetric in \(x\) and \(y\).

\paragraph{Proposition}\label{hit-equivalence}

\(V ≃ M/≈\)

\emph{Proof:} Direct consequence of the previous two lemmas.

\paragraph{Remark}\label{remark}

That \(M/≈\) is equivalent to the HIT formulation in the book can be
seen from Lemma 10.5.5 of ``Homotopy Type Theory''\footcite{hottbook}.
Thus, proposition \ref{hit-equivalence} shows that our \(V\) is indeed
equivalent to the HIT formulation of \(V\).


==> iterative-sets/id-models.tex <==
\section{Models where equality is
identity}\label{models-where-equality-is-identity}

In this section we define what an ∈-structure is, and give some basic
results on such structures in generality. We do this in order to adjust
our expectation for the concrete model which will be main focus of this
work.

\subsection{∈-structures}\label{structures}

\paragraph{Definition}\label{definition}

An \emph{∈-structure} is a pair \((ℳ,∈)\) where \(ℳ : \Set\) is a mere
set, and \(∈ : ℳ → ℳ → \Prop\).

\paragraph{Definition}\label{definition-1}

For any ∈-structure \((ℳ,∈)\) and element \(a : ℳ\), we define
\(E␣a ≔ ∑_{x : ℳ} x∈a\).

\paragraph{Definition}\label{definition-2}

An ∈-structure \((ℳ,∈)\) is called \emph{\(U\)-like} if for each
\(a : ℳ\) the type \(E␣a\) is essentially \(U\)-small. That is, if each
\(a : ℳ\) the type \(E␣a\) has a code in \(U\).

\paragraph{Remark}\label{remark}

An ∈-structure is basically a mere set with a merely propositional,
binary predicate defined on it. The natural equality to consider for
elements of such a structure is the identity type. This is in contrast
to the setoid approach taken by Aczel.

``\(U\)-like'' is meant to mimic the traditional terminology,
``set-like'', used in set theory.

\subsection{Translations of first-order logic into type
theory}\label{translations-of-first-order-logic-into-type-theory}

\paragraph{Definition}\label{definition-3}

Given an ∈-structure \((ℳ,∈)\) define two translations of formulas of
first-order logic to type theory, \(σ_{ℳ,∈}\) and \(τ_{ℳ,∈}\), by
recursion on formulas. We let \(\Ctx\) denote contexts (finite lists of
variables, \(\Vars␣Γ\) denoting the variables in \(Γ\)) and let
\(\Fml␣Γ\) denote formulas in a given context \(Γ : \Ctx\).

Starting with \(σ_{ℳ,∈}\), leaving out the subscripts for ease of
reading:

\begin{align*}
  σ &: ∏_{Γ:\Ctx} \Fml␣Γ → (\Vars␣Γ → ℳ) → \Type \\
  σ &␣Γ␣(∀x\ φ)␣γ := ∏_{a:ℳ} σ␣(Γ.x) φ␣(γ.a) \\
  σ &␣Γ␣(∃x\ φ)␣γ := ∑_{a:ℳ} σ␣(Γ.x) φ␣(γ.a) \\
  σ &␣Γ␣(φ∧ψ)␣γ := σ␣Γ␣φ␣γ × σ␣Γ␣ψ␣γ \\
  σ &␣Γ␣(φ∨ψ)␣γ := σ␣Γ␣φ␣γ + σ␣Γ␣ψ␣γ \\
  σ &␣Γ␣(φ→ψ)␣γ := σ␣Γ␣φ␣γ → σ␣Γ␣ψ␣γ \\
  σ &␣Γ␣⊥␣γ := 0 \\
  σ &␣Γ␣⊤␣γ := 1 \\
  σ &␣Γ␣(x ∈ y)␣γ := γ␣x ∈ γ␣y\\
  σ &␣Γ␣(x = y)␣γ := γ␣x =_{ℳ} γ␣y
\end{align*}

\noindent where \(Γ.x\) denotes the context \(Γ\) extended with the
variable \(x\), and \(γ.a\) denotes the function \(\Vars␣(Γ.x) → ℳ\)
which maps \(x\) to \(a\).

We define \(τ_{ℳ,∈}\) analogously, only difference being in the clauses
for ∨ and ∃:

\begin{align*}
  τ &: ∏_{Γ:\Ctx} \Fml␣Γ → (\Vars␣Γ → ℳ) → \Type \\
  τ &␣Γ␣(∀x\ φ)␣γ := ∏_{a:ℳ} τ␣(Γ.x) φ␣(γ.a) \\
  τ &␣Γ␣(∃x\ φ)␣γ := ∃(a:ℳ)\ τ␣(Γ.x) φ␣(γ.a) \\
  τ &␣Γ␣(φ∧ψ)␣γ := τ␣Γ␣φ␣γ × τ␣Γ␣ψ␣γ \\
  τ &␣Γ␣(φ∨ψ)␣γ := τ␣Γ␣φ␣γ ∨ τ␣Γ␣ψ␣γ \\
  τ &␣Γ␣(φ→ψ)␣γ := τ␣Γ␣φ␣γ → τ␣Γ␣ψ␣γ \\
  τ &␣Γ␣⊥␣γ := 0 \\
  τ &␣Γ␣⊤␣γ := 1 \\
  τ &␣Γ␣(x ∈ y)␣γ := γ␣x ∈ γ␣y\\
  τ &␣Γ␣(x = y)␣γ := γ␣x =_{ℳ} γ␣y
\end{align*}

\paragraph{Example}\label{example}

The axiom of union is translated differently by the two translations:

\begin{align*}
 \UNION ≔& ∀x␣∃u␣∀z\ z∈u ↔ ∃y∈x␣z∈y \\
 σ␣()␣(\UNION)
   =& ∑_{u:ℳ} ∏_{z:ℳ} z∈u ↔ ∑_{y : ℳ} y∈x ∧ z ∈ y \\
 τ␣()␣(\UNION)
   =& ∃(u:ℳ)\ ∏_{z:ℳ} z∈u ↔ ∃(y : ℳ)\ y∈x ∧ z ∈ y
\end{align*}

If the structure \((ℳ,∈)\) satisfies the extensionality axiom, then the
property \(∏_{z:ℳ} z∈u ↔ ∃(y : ℳ)\ y∈x ∧ z ∈ y\) completely
characterises \(u\), making
\(τ␣()␣(\UNION) ≃ ∑_{u:ℳ} ∏_{z:ℳ} z∈u ↔ ∃(y : ℳ)\ y∈x ∧ z ∈ y\).
However, \(∑_{y : ℳ} y∈x ∧ z ∈ y\) is not always implied by
\(∃(y : ℳ)\ y∈x ∧ z ∈ y\) so the two axioms remain distinct.

\subsection{Axioms of set theory}\label{axioms-of-set-theory}

The axioms of set theory contain a number of axiom schemas, such as
collection or replacement, or (restricted) separation. In set theory
this adds one axiom for each first-order formula. In type theory it is
more convenient to use the higher order features of type theory and
regard these as quantified over all predicates. The result is much
stronger than the original axiom scheme. In the following we will
exploit this extra strength.

\paragraph{Definition}\label{definition-4}

Given a structure, \((ℳ,∈)\), and a predicate \newline
\(P : ℳ → ℳ → \Type\) and an element \(m : ℳ\), we define
\emph{σ-replacement for \(P\) and \(m\) in \((ℳ,∈)\)} to be the type
\newline
\(σ_{P}␣(a)␣((∀x∈a␣∃!y\ P␣x␣y)→∃b␣∀y(y∈b ↔ ∃x∈a\ P␣x␣y))␣m\), where
\(σ_{P}\) is \(σ\) extended with the clause
\(σ␣Γ␣(P␣x␣y)␣γ ≔ P␣(γ␣x)␣(γ␣y)\), in order to interpret the \(P\) as a
predicate symbol.

Define τ-replacement in the same way, substituting τ for σ.

\paragraph{Proposition}\label{proposition}

\label{ac-from-replacement}

If an ∈-structure \((ℳ,∈)\) satisfies extensionality, σ-replacement and
has an ordered pairing operation \(〈-,-〉 : ℳ → ℳ → ℳ\), then the
following choice principle, stemming from the so-called \emph{type
theoretic choice principle}\footnote{The type theoretic choice principle
  is the fact that for all \(A\), \(B\) and \(P\), the type
  \(\left(∏_{a:A}∑_{b:B␣a}P␣a␣b\right) → ∑_{f:∏_{a:A}B␣a}∏_{a:A}P␣a␣(f␣a)\)
  is inhabited.}, holds:

For any \(P : ℳ → ℳ → \Type\) and \(a,b : ℳ\) if

\begin{align*}
∏_{x : ℳ} x∈a → ∑_{y : ℳ} {y∈B}∧{P␣x␣y}\text{,}
\end{align*}

\noindent then there is a function \(f : ℳ\) with domain \(a\) and
codomain \(b\) such that \(∏_{x : ℳ} P␣x␣(f␣x)\).

\emph{Proof:} Given \(a\),\(b\) and a proof
\(p : ∏_{x : ℳ} x∈a → ∑_{y : ℳ} {y∈B}∧{P␣x␣y}\), apply σ-replacement to
\(a\) and the predicate \(P' : ℳ → ℳ → \Prop\) defined by

\begin{align*}
 P'␣x␣z &≔ ∑_{q : x ∈ a} z =_ℳ {〈x,π₀␣(p␣x␣q)〉}
\end{align*}

The resulting element of \(ℳ\) is a function with the desired
properties.∎

\paragraph{Remark}\label{remark-1}

Proposition \ref{ac-from-replacement} shows us that we cannot hope to
have a model satisfying all axioms of constructive set theory by
interpreting the existential quantifier as Σ-types while at the same
time interpreting equality as the identity type of a mere set. This is
because the above proposition shows that AC will hold, in this
interpretation, and thus if all other CZF axioms hold (in fact
\(U\)-restricted separation and pairing should suffice), Diaconescu's
theorem demonstrates that the law of excluded middle holds (for all
\(U\)-small propositions).


==> iterative-sets/introduction.tex <==
\section{Introduction}\label{introduction}

The first model of set theory in type theory is due to Aczel and models
the constructive set theory CZF\footcite{aczel1978}. The underlying type
of sets in this model is \(W_U T\), the type of all well-founded trees
with branchings in a universe \(U\) with decoding family
\(T : U → {\Type}\). The interpretation of equality in this model allows
deduplication and permutation of subtrees --- incorporating the
intuition that the order and multiplicity of elements of a set are
irrelevant. If we instead insist to interpret equality as the identity
type and assume the univalence axiom, the underlying type no longer
models set theory, but rather multiset theory.

In a related work\footnote{\multisetsref} we explore the notion of
iterative multisets in type theory. Here we will specialise from the
general multisets to the set-like ones, where each element occurs at
most once. We will start by summarising the model of multisets and its
relation to Aczel's model of CZF in type theory\footcite{aczel1978}.

Once the notion of a multiset is defined, it is natural to study the
hereditary subtype of multisets where each element occurs at most once.
These are in a certain sense the most natural representations of
iterative sets from a homotopy type theory point of view. These are
namely the multisets for which the element hood relation is
hereditarily, merely propositional (type level −1).

In this text we explore how this type models various axioms of
constructive set theory. We also show that it is equivalent to the
higher inductive type outlined in the book ``Homotopy Type Theory''
\footcite{hottbook}.

\subsection{From multisets to sets -- two
ways}\label{from-multisets-to-sets-two-ways}

Assume for a moment that we would like to explain the notion of multiset
to someone who knows the notion of a set. Here are two similar attempts
at such an explanation.

\subsubsection{Variant A}\label{variant-a}

\begin{quote}
A multiset is a generalisation of sets in which an element may occur any
number of times, not just at most once.
\end{quote}

\subsubsection{Variant B}\label{variant-b}

\begin{quote}
A multiset is like a set with the extra information attached to each
element about how many times it occurs in the multiset.
\end{quote}

The two descriptions are almost identical, but critically different.
Variant A describes the multisets as a more general concept than sets,
in the sense that a set is a \emph{special case} of a multiset, namely
those multisets in which each element occurs at most once. Variant B, on
the other hand, describes a multisets as sets with some extra structure.
In both cases the impression given is that the multisets are, in an
informal way, a \emph{bigger concept} than that of a set. Variant A says
that sets are just some of the multisets, while Variant B says that for
each set there are numerous ways to make a multiset from it.

In mathematics these two notions of ``bigger'' correspond to the notion
of

\begin{itemize}
\itemsep1pt\parskip0pt\parsep0pt
\item
  sets being a subtype of multisets (Variant A)
\item
  sets being a quotient of multisets (Variant B)
\end{itemize}

If we were to turn the direction of explanations, making them
explanations of the concept of a set from the notion of a multiset, the
above suggests two distinct routes of constructing a notion of sets from
a notion of multisets. We either identify the subtype of \emph{set-like}
multisets, or identify the equivalence relation of multisets which
\emph{forgets the extra structure of multiplicites}.

\paragraph{Example}\label{example}

The multiset \(\{a,a,b\}\) would not be considered a set-like in the
spirit of Variant A, since \(a\) occurs twice. On the other hand,
Variant B would contest that \(\{a,a,b\}\) and \(\{a,b,b\}\) would
\emph{represent the same} set, since in both cases \(a\) and \(b\) are
exactly the elements occurring at least once. \vspace{3mm}

If we denote by \(M\) the multisets, and \(V_A\) and \(V_B\) denotes the
two possible notions of sets arising from it, following Variant A and
Variant B respectively, we can draw the following diagram of the
situation.

\begin{align*}
\xymatrix{
V_A \ar@{^{(}->}[r] & M \ar@{->>}[d] \\
  & V_B
}
\end{align*}

\subsection{Outline}\label{outline}

In Section 2 and 3 we set up a bit of framework to work within. Starting
from Section 4 we will follow the path of Variant A.

Section 5 will take us through the basic lemmas about the type of
iterative sets we define in Section 4. These lemmas are applied in
Section 6 to give proofs that our model satisfies the axioms of Myhill's
Constructive Set Theory.

In Section 7 we consider the problem of interpreting the two collection
axioms of Aczel's CZF in our model.

In Section 8 we return to Variant B, which will make the relationship
with the approach taken in Chapter 10 of the book ``Homotopy Type
Theory''\footcite{hottbook} clear.

\subsection{Notation}\label{notation}

In what follows we will adhere to the following notation. Some of our
notation is similar to that of the book ``Homotopy Type Theory''
\footcite{hottbook}, while some of it is inspired by the syntax of Agda.

\begin{itemize}
\itemsep1pt\parskip0pt\parsep0pt
\item
  Function application will be denoted by juxtaposition, as in \(f␣a\).
  Also, application of functions equipped with extra structure, such as
  equivalences and embeddings, will be denoted by juxtaposition.
\item
  Quantifiiers, such as ∀,∃,∏ and ∑ bind weakly. For instance, \newline
     \(∏_{x : ℳ} x∈a → ∑_{y : ℳ} {y∈B}∧{P␣x␣y}\) disambiguates
  to\newline
     \(∏_{x : ℳ} \left(x∈a → ∑_{y : ℳ} {y∈B}∧{P␣x␣y}\right)\)
\item
  The equality sign, \(=\), denotes the identity type. We sometimes
  equip it with a subscript emphasising which type the elements belong
  to, as in \(a =_A a'\).
\item
  Definitions are signified by \(≔\).
\item
  Judgemental equalities are denoted by \(≡\).
\item
  The notation \(A : \Type\) denotes that \(A\) is a type,
\item
  The notation \(A : \Set\) denotes that \(A\) is a type which is a mere
  set and
\item
  The notation \(A : \Prop\) denotes that \(A\) is a type which is a
  mere proposition.
\item
  The type \(U\) is a universe, with decoding family \(T : U → \Type\).
  We assume that this universe

  \begin{itemize}
  \itemsep1pt\parskip0pt\parsep0pt
  \item
    is univalent,
  \item
    contains the empty type, \(0\),
  \item
    is closed under Π-types,
  \item
    is closed under Σ-types,
  \item
    is closed under \(+\)-types,
  \item
    is closed under \((-1)\)-truncation and
  \item
    is closed under taking quotients of mere sets by equivalence
    relations.
  \end{itemize}
\item
  The notation \(e_A\) denotes the empty function \(e : 0 → A\). The
  subscript is dropped when inferable from the context.
\item
  The notation \(ap␣f\) refers to the usual function
  \(\ap␣f : a = a' → f␣a = f␣a'\)
\end{itemize}


==> iterative-sets/lemmas.tex <==
\section{Basic results}\label{basic-results}

In this section we clarify the basic properties of iterative multisets
and \newline \((V, ∈_V)\). The most important of these is the
extensionality of \(V\) with respect to \(∈_V\).

We start with reminding ourselves of the extensionality theorem for
multisets.

\paragraph{Theorem}\label{theorem}

\(x =_M y ≃ ∏_{z : M} \left( \left(z ∈_M y\right) ≃ \left(z ∈_M y\right)\right)\)

\emph{Proof:} See Theorem \ref{multiset-extensionality} in Subsection
\ref{multiset-extensionality-section} of \multisetsref.

\paragraph{Lemma}\label{lemma}

The type \(\itset␣x\) is a mere proposition for every \(x : M\).

\emph{Proof:} Immediate by induction on \(M\) and that \(\embedding f\)
is a mere proposition.

\paragraph{Lemma}\label{lemma-1}

The function \(\ap␣π₀ : (x =_V y) → (π₀␣x =_M π₀␣y)\) is an equivalence.

\emph{Proof:} Simple consequence of \(\itset\) being a mere proposition.

\paragraph{Lemma}\label{lemma-2}

For any \(x: M\) and \(y : V\) we have that the type \(x ∈_M π₀y\) is a
mere proposition.

\emph{Proof:} Assume \(y ≡ (\sup␣a␣f , (p , q))\). Observe that
\(x ∈_M π₀y\) is the fibre of \(f\) over \(y\). Since \(p\) proves \(f\)
to be an embedding, and embeddings have propositional fibres, then
\(x ∈_M π₀y\) is a proposition.∎

\paragraph{Lemma}\label{lemma-3}

\begin{align*}
\left(∏_{z : V} \left(z ∈_V x ↔ z ∈_V y\right)\right)
≃ \left(∏_{z : M} \left(z ∈_M π₀x ↔ z ∈_M π₀y\right)\right)
\end{align*}

\emph{Proof:} Both sides of the equivalence are mere propositions, so it
is enough to show biimplication. Passing from right to left is trivial,
so we show only the implication from left to right.

Assume \(z : M\). If \(z ∈ π₀x\) then \(z\) must be an iterative set.
Thus, \(z ∈ y\) which is to say \(z ∈ π₀y\). This demonstrates
\(z ∈ π₀x → z ∈ π₀y\). That \(z ∈ π₀y → z ∈ π₀x\) is shown
symmetrically. Hence, \(z ∈ π₀x ↔ z ∈ π₀y\), which completes the proof.∎

\paragraph{Lemma}\label{lemma-4}

\label{image-lemma} Given a small type \(a : U\) and a function
\(f : T␣a → V\), there is a set \({\image}␣a␣f\) such that

\begin{itemize}
\itemsep1pt\parskip0pt\parsep0pt
\item
  for each \(i : T␣a\) we have that \(f␣i ∈ ({\image}␣a␣f)\)
\item
  for any merely propositional predicate \(P : V → \Set\),
  given\hfill\newline
  \(∏_{i : T␣a} P␣(f␣i)\) we can prove that
  \(∏_{z : V} (z ∈ ({\image}␣a␣f) → P␣z)\).
\end{itemize}

\emph{Proof:} Given \(a : U\) and \(f : T␣a → V\). Take the image
factorisation of \(f\), which can be expressed as a simple higher
inductive type. Since \(V\) is locally \(U\)-small, the image has a code
\(b : U\). Denote the injection of the image into \(V\) by
\(g :T b → V\), and define \(\image␣a␣f := \sup␣b␣v\). ∎


==> iterative-sets/model.tex <==
\section{The model of iterative sets}\label{the-model-of-iterative-sets}

We recall the definition, from \multisetsref, of the type of iterated
multisets and the membership relation.

\paragraph{Definition}\label{definition}

\begin{align*}
M ≔ W_UT
\end{align*}\begin{align*}
&∈_M : M → M → \Set \\
x &∈_M (\sup␣a␣f) ≔ ∑_{i:T␣a} f␣i = x
\end{align*}

The elements of \(M\) are the iterative multiset in which another
element of \(M\) may occur any \(U\)-small number of times. This is
expressed by the relation \(∈_M\), as follows: Given \(x,y : M\) the
type \(x ∈_M y\) is the type of occurrences of \(x\) in \(y\). For
instance, if \((x ∈_M y) ≃ 2\) then \(x\) occurs twice in \(y\).

What we would like to consider are the elements of \(M\) in which every
element occurs at most once. Such a multiset would be called
\emph{set-like}. Being set-like could be expressed in different ways.
The most direct would be to say that \(y : M\) is set-like whenever
\(x ∈_M y\) is a mere proposition for all other \(x : M\). Another way
to state this is to say that the function mapping each instance of an
element in \(y\) to the element it represents is an embedding.

The \emph{iterative sets} are those multisets which are hereditarily
set-like. On \(M\) we define the predicate \(\itset\), recursively, as
follows.

\paragraph{Definition}\label{definition-1}

\begin{align*}
&\itset : M → \Type \\
&\itset␣(\sup␣a␣f) ≔ \embedding␣f ∧ ∏_{i : T␣a} \itset␣(f␣a)
\end{align*}

For each \(x : M\), whenever we have \(\itset␣x\), we say that \(x\) is
an \emph{iterative set}.

A Σ-type then collects the type of iterative sets as a subtype of \(M\)
-- with elementhood defined by the restriction of elementhood for
multisets.

\paragraph{Definition}\label{definition-2}

The type of iterative sets, \(V\), is defined as the subtype of \(M\) of
iterative sets, or \(V ≡ ∑_{x:M} \itset␣x\).

We denote by \(∈_V\) the specialisation of \(∈_M\) to \(V\), that
is\newline
\(x ∈_V y ≔ π₀␣x ∈_M π₀␣y\).

\paragraph{Notation}\label{notation}

We will permit ourselves a slight abuse of notation when denoting
elements of \(V\). We will for the remainder of this article use the
notation \(\sup␣a␣f\) to denote an element of \(V\) constructed by
\(a : U\) and an embedding \(f : T␣a ↪ V\).

\paragraph{Remark}\label{remark}

Checking that a multiset is an iterative set can be a tedious task,
since it has to be carried out on each level, but the next section will
give lemmas to make it easier to construct new iterative sets.


==> iterative-sets/myhill.tex <==
\section{V models Myhill's constructive set
theory}\label{v-models-myhills-constructive-set-theory}

In this section we prove that \((V , ∈_V)\) models the axioms of
Myhill's Constructive Set Theory (CST), when the existential quantifiers
are interpreted as truncated. In fact, we shall see that except for a
few critical places, positive occurrences of the existential quantifier
can be strengthened to ∑, mostly because the constructions we make are
explicit.

\subsection{Extensionality}\label{extensionality}

The lemmas we have proved line up to give the following equivalence:

\paragraph{Extensionality}\label{extensionality-1}

\(x =_V y ↔ ∏_{z : V} \left(z ∈ x ↔ z ∈ y\right)\)

\emph{Proof:}

\begin{align}
 x =_V y &≃ π₀x = π₀ y \\
         &≃ ∏_{z : M} \left(z ∈_M π₀x ≃ z ∈_M π₀y\right) \\
         &≃ ∏_{z : M} \left(z ∈_M π₀x ↔ z ∈_M π₀y\right) \\
         &≃ ∏_{z : V} \left(z ∈_V π₀x ↔ z ∈_M π₀y\right)
\end{align}

∎

\subsection{The empty set, natural
numbers}\label{the-empty-set-natural-numbers}

The empty set is given by \(∅ ≔ \sup 0 e\). The natural numbers we
constructed in \multisetsref, Subsection \ref{natural-numbers-multiset}
is indeed an iterative set.

\subsection{Separation}\label{separation}

Restricted separation can be done in \(V\) without quotienting, as long
as the separating predicate is merely propositional. Thus, whenever we
separate a formula with existential quantifier in a positive position,
the existence must be unique or truncated. If there are more than one
witness of the statement, the result would be a multiset where the
element occurs once per witness of the statement. The same is true for
disjunction. Notice that if \(A + B\) is a proposition then \(A\) and
\(B\) are mutually exclusive (since \(l␣a\) and \(r␣b\) are always
distinct).

\paragraph{Proposition}\label{proposition}

For any \(U\)-small predicate \(P : V i → \Prop\), and \(x : V\) there
is \(u : V\) such that for any \(z : V\) we have
\(z ∈ u ↔ (P␣z) × (z ∈ x)\).

\emph{Proof:} Assume that \(x≡\sup␣A␣f\) and let
\(u ≔ \sup (∑_{a : A} P␣(f␣a)) (f ∘ π₀)\). Since \(P∘f\) is a mere
proposition \(π₀ : (∑_{a : A} P␣(f␣a)) → A\) is injective, thus
\(f ∘ π₀\) is injective.

If \(z ∈ u\) then \(z = f␣a\) for some \(a : A\) such that \(P␣(f␣a)\),
and hence \(P␣z\) and \(z ∈ x\).

If \(p:P␣z\) and \(q:z ∈ x\) then let \(a ≔ π₀ q\), \(((a,p),π₁␣q)\)
will prove that \(z ∈ u\).∎

\subsubsection{∈-induction}\label{induction}

Induction on \(V\) can be performed, even when the predicate is a
general type, not necessarily merely propositional.

\paragraph{Proposition}\label{proposition-1}

For every predicate \(P : V → \Type\), if for each \(x : V\) we have
that \(∏_{y : V} y ∈ x → P␣y\) implies \(P␣x\), then we have \(P␣x\) for
every \(x : V\).

\emph{Proof.} By induction on \(V\). Assume \(x ≡ \sup␣A␣f\) then by
induction hypothesis \(P␣(f␣i)\) for every \(i : A\). We must show that
if \(y ∈ x\) then \(P␣y\). However, \(y ∈ x\) means that there is \(i\)
such that \(y = f␣i\) so we can transport the induction hypothesis to
obtain \(P␣y\). Thus, we have shown \(∏_{y : V} y ∈ x → P␣y\), which
implies \(P␣x\) by assumption.∎

\subsection{Pairing and Union}\label{pairing-and-union}

In order to show pairing and union we will have to apply the image
construction, previously introduced (Lemma \ref{image-lemma}). If we
applied the constructions of union and pairing for multisets which we
defined in \multisetsref, then the resulting multisets would not be
set-like. Therefore, we need a different construction, and the most
natural is to take quotients to make the multisets back into sets. The
fact that quotienting was not needed for multisets, may be an indication
that iterative multisets is a more natural notion than iterative sets to
consider in type theory.

\paragraph{Definition}\label{definition}

Given \(x,y : V\), we define
\(\{x,y\} ≔ \image␣(1 + 1)␣(\const x + \const y)\).

\paragraph{Proposition}\label{proposition-2}

For any \(x,y : V\) and for each \(z : V\) we have that
\(z ∈ \{x,y\} ↔ ((x = z) ∨ (y = z))\)

\emph{Proof:} Simple consequence of Lemma \ref{image-lemma}.∎

\paragraph{Definition}\label{definition-1}

Given \(x : V\), where \(x ≡ \sup␣A␣f\) define

\(∪ x ≔ {\image}␣(∑_{a:A} (\overline{f␣a}))␣  (λ〈i,j〉. \widetilde{(f i)} j)\).

\paragraph{Proposition}\label{proposition-3}

For any \(x : V\) and for any \(z : V\), we have that
\(z ∈ ∪x ↔ ∃y\ ({y ∈ x} ∧ {z ∈ y})\)

\emph{Proof:} Simple consequence of Lemma \ref{image-lemma}.∎

\paragraph{Remark}\label{remark}

The truncated existential quantifier in the above proposition cannot be
strengthened to a Σ-type, since it would mean constructing sections for
almost arbitrary quotients.

\subsection{Replacement}\label{replacement}

\paragraph{Proposition}\label{proposition-4}

\label{replacement}

For any \(a : V\) and \(P : V → V → \Prop\), such that for all \(x ∈ a\)
there exists a unique \(y\) for which \(P␣x␣y\), then there is \(b : V\)
such that for each \(y : V\) we have that \(y ∈ b\) if and only if there
exists \(x ∈ a\) such that \(P␣x␣y\).

\emph{Proof:} Given \(a = \sup␣\bar a␣\tilde a\), the assumptions let us
construct a map \(T␣\bar a → V\). Using Lemma \ref{image-lemma}, we can
construct its image in \(V\), which will have the desired properties.∎

\paragraph{Proposition}\label{proposition-5}

For any \(a : V\) and \(F : V → V\), there is \(y : V\) such that for
any \(z : V\) we have \(z ∈ b ↔ ∃(w : V)\ z = F␣w\).

\emph{Proof:} Assume \(x ≡ \sup␣a␣f\) and let \(b = \image␣(F∘f)\), and
apply Lemma \ref{image-lemma}.∎

\subsection{Exponentials}\label{exponentials}

The construction of exponentials in this model is particularly easy,
since a set-theoretical function between two elements, \((\sup␣A␣f)\)
and \((\sup␣B␣g)\), of \(V\) boils down to a function in the type theory
\(A → B\). Instead of giving a direct proof, we can lean on
\multisetsref, Subsection \ref{multiset-exp} in order to prove the
correctness of this construction.

\subsubsection{Exponentiation}\label{exponentiation}

Exponentiation of sets is a special case of exponentiation of multisets.
For multisets, we defined\footnote{Definition \ref{operation-definition}
  in Subsection \ref{multiset-functions} of \multisetsref}\(\operation_{a,b}␣f\)
for every \(a,b,f : M\), and showed that there is a multiset
\(\Exp␣a␣b\), such that\newline
\({f ∈ \Exp␣a␣b} ≃\operation_{a,b}␣f\). We will here show that whenever
\(a,b,f: V\), we have \(\operation_{π₀␣a,π₀␣b}␣(π₀␣f)\) if an only if
\(\Fun␣a␣b␣f\), and that in fact \(\itset␣(\Exp␣(π₀␣a)␣(π₀␣b))\), in
order to conclude that there is exponentiation in \(V\).

\paragraph{Lemma}\label{lemma}

\label{exp-lemma1}

Whenever \(a,b,f: V\), we have that\newline
\(\operation_{π₀␣a,π₀␣b}␣(π₀␣f) ↔ \Fun␣a␣b␣f\).

\emph{Proof:} Recall that\footnote{ibid.} for every \(a,b,f : M\),

\begin{align*}
\operation_{a␣b}␣f ≔ &\left(∏_z␣z ∈ f → ∑_x␣∑_y␣z=〈 x , y 〉 \right) \\ 
                   ∧ &\left(∏_x␣x ∈ a ≃ ∑_y 〈 x , y 〉 ∈ f \right) \\
                   ∧ &\left(∏_y␣y ∈ b ← ∑_x 〈 x , y 〉 ∈ f \right) 
\end{align*}

If here it said \(↔\) instead of \(≃\), this would state that \(f\) is a
total relation between \(a\) and \(b\). We thus have to show that this
strengthening is exactly the same as ensuring functionality of a total
relation.

In the middle conjunction, \(x∈a\) is a mere proposition since \(a\) is
an iterative set by assumption. Thus, \(∑_y 〈 x , y 〉 ∈ f\) must also
be a mere proposition, and thus equivalent to
\(∃!(y:M) 〈 x , y 〉 ∈ f\). This is exactly the requirement for a total
relation to be functional.∎

\emph{Remark:} Since \(\operation_{π₀␣a,π₀␣b}␣(π₀␣f)\) and
\(\Fun␣a␣b␣f\) are both mere propositions, the biimplication is also an
equivalence of types.

\paragraph{Lemma}\label{lemma-1}

\label{exp-lemma2}

For every \(a, b : V\) the multiset \(\Exp␣(π₀␣a)␣(π₀␣b)\) is an
iterative set.

\emph{Proof:} The definition of \(\Exp␣a␣(π₀ b)\) is\ldots{}

\begin{align*}
\operatorname{Exp}␣(π₀ a)␣(π₀ b) := 
                   \sup␣&(\overline{(π₀␣a)}→ \overline{(π₀␣b)}) \\
                        ␣&(λf. \sup␣\overline{(π₀␣a)} \\
                        ␣&(λi. 〈 \widetilde{(π₀␣a)} i
                              , \widetilde{(π₀␣b)}␣(f␣i)〉))
\end{align*}

Thus, we need to show that the function \newline
\(λf. \sup␣\overline{(π₀␣a)}␣(λi. 〈 \widetilde{(π₀ a)} i , \widetilde{(π₀ b)} (f␣i) 〉)\),
which takes a function to its graph, is injective, but this comes down
to that a function is determined by its graph, which follows from
function extensionality.

Next, we need to argue that each graph of each function is itself an
iterative set. Assume that
\(f : \overline{(π₀␣a)} → \overline{(π₀␣b)}\), then the function which
maps an element \(i : \bar (π₀ a)\) to
\(〈 \widetilde{(π₀ a)}␣i , \widetilde {(π₀ b)}␣(f i) 〉\) is injective
since \(π₀␣a\) is an iterative set. Furthermore,
\(〈 \widetilde {(π₀␣a)}␣i , \widetilde{(π₀␣b)}␣(f␣i) 〉\) is an
iterative set since both \(a\) and \(b\) are iterative sets. Thus, the
graph of \(f\) is an iterative set.∎

\paragraph{Proposition}\label{proposition-6}

For every \(a,b : V\) there is a \(u : V\) such that for any \(c : V\)
there is an biimplication \(c ∈ u ↔ \Fun␣a␣b␣c\).

\emph{Proof:} Direct from Lemma \ref{exp-lemma1}, Lemma
\ref{exp-lemma2}, and exponentiation in \(M\)\footnote{\texttt{(M-EXP)}
  in Subsection \ref{multiset-exp}, \multisetsref}, letting
\(u ≔ \Exp␣(π₀ a)␣(π₀ b) ↔ \Fun␣a␣b␣f\).∎


==> iterative-sets/notes <==
IAAC Aczel (1973 strength of martin löf type theory)


Collection
==========


   A : Set(U) , B : Type    P : A × B → Prop
──────────────────────────────────────────────────────────────────
  ∏ (a : A) ∃ (b : B)  P x y  → ∃ (C : U) (f : C ->> A) (g : C → B) ∏ (c : C) P (f c) (g c)


## Example: Multiset of roots of a polynomial

Let $f : ℝ[x]$ be some real polynomial. Then let us specify a multiset
by letting 

$I_f ≔ ∑_{x₀ : ℝ} ∑_{n:ℕ}\ (x - x₀)^{n+1} | f$ 

be our set of occurences,
and $p_f ≔ π₀$ associate each occurence with its element in $ℝ$.

This is the multiset of roots of $f$.


==> iterative-sets/types.tex <==
\section{Types and propositions}\label{types-and-propositions}

One of the main features of Martin-Löf's type theory is the
interpretation of propositions as types\footcite{mltt}. The presence of
the identity type gives the possibility of asking whether two proofs of
a proposition are equal. A type in which all elements are equal is
called, in homotopy type theory, a \emph{mere proposition}.

The traditional interpretation of the existential quantifier in type
theory is by the sigma type \(∑_{a : A} P␣a\). A proof of an existential
proposition is thus \(a , p\) --- a term \(a : A\) of the quantified
domain paired with a proof \(p : P␣a\) that the term has the correct
property. It is clear that since the existence is not necessarily
unique, the type of such proof need not be a mere proposition.

In homotopy type theory, one introduces a truncated existential
quantifier \(∃(x:A) P␣a\), which is constructed from \(∑_{a : A} P␣a\)
by adding identifications of all elements in to make it a mere
proposition. This gives the following introduction and elimination
rule:\footnote{In these rules, written in an Agda-like notation,
  \texttt{Prop} refers to the type of mere propositions.}

\begin{verbatim}
   a : A     b : B a
─────────────────────── ∃-intro
     [a,b] : ∃(a:A)(B a)

   x : ∃(a:A)(B a)   y : ∃(a:A)(B a)
────────────────────────────────── ∃-quot
     q : x = y

  P : ∃(a:A)(Ba) → Prop  
  p : (a : A) → (b : B a) → P [a,b]
──────────────────────────────────────────── ∃-elim
     ∃-elim P p : (x : ∃(a:A)(B a)) → P x
\end{verbatim}

Clearly \(∑_{a:A}(B␣a) → ∃(a:A)(Ba)\) holds for all \(A\) and \(B\). The
opposite implication holds if \(∑_{a:A}(B␣a)\) is a mere proposition --
which is to say that the existence is unique, with a unique proof.

The situation is similar for disjunctions. Traditionally, disjunction is
interpreted as disjoint union in Martin-Löf's type theory, while
homotopy type theory introduces a truncated variant. We will denote
disjoint unions by the operator \(+\) and the truncated disjunction by
the operator \(∨\).


==> multisets/abstract.tex <==
\begin{abstract}
A multiset consists of elements, but the notion of a multiset is distinguished
from that of a set by carrying information of how many times each element
occurs in a given multiset. In this work we will investigate the notion of
iterative multisets, where multisets are iteratively built up from other
multisets, in the context Martin-Löf Type Theory, in the presence of
Voevodsky’s Univalence Axiom.

\cite{aczel1978} introduced a model of constructive set theory in type theory,
using a W-type quantifying over a universe, and an inductively defined
equivalence relation on it. Our investigation takes this W-type and instead
considers the identity type on it, which can be computed from the Univalence
Axiom. Our thesis is that this gives a model of multisets. In order to demonstrate
this, we adapt axioms of constructive set theory to multisets, and show that
they hold for our model.
\end{abstract}



==> multisets/constructions.tex <==
\section{Multiset constructions}

Aczel's $V$ is a model of CZF. To mirror this we look at axioms of constructive
set theory, and attempt to find corresponding axioms for multisets. The main
observation is that definite axioms\footnote{An axiom is \emph{definite} if any set
it claims existence of is characterised uniquely.} can be systematically
changed to axioms which makes
sense for multisets, by carefully strengthening logical equivalence, $↔$, to
equivalence in type theory $≃$. A feature of this conversion is that for the
axioms below, we can retain the constructions from Aczel's $V$ when we prove that
the changed axioms hold for $M$.


The axioms we will have a look at are

\begin{itemize}
\item
  Extensionality
\item
  Restricted separation
\item
  Union Replacement
\item
  Pairing \& singletons
\item
  Infinity.
\item
  Exponentiation / Fullness
\item
  Collection.
\end{itemize}


\subsection{Restricted separation}
The axiom of restricted separation says that we can select subsets by use of
formulas, as long as they are bounded. For multisets, this corresponds to
that we may multiply the number of occurrences by the family of sets represented
by the formula, as long as the family is $U$-small.

\begin{align*}
\mathtt{(RSEP)}& & ∀ x ∃ u ∀ z \left(z ∈ u ↔ \left( z ∈ x ∧ P \right) \right)
\end{align*}
where $P$ is a restricted formula where $u$ does not occur freely in $P$.

The formulation of \texttt{RSEP} in first order logic can be translated into
type theory, given our domain $M$, replacing ↔ with ≃.


\begin{proposition}
\begin{align*}
\mathtt{(M-RSEP)}& &∏_{x : M} ∑_{u : M} ∏_{z : M} \left(z ∈ u ≃ \left( z ∈ x ∧ T␣(P␣z) \right) \right),
\end{align*}
where $P : M → U$, is a $U$-small family.
\end{proposition}

\begin{proof}
Define
\begin{align}
&\operatorname{Sep} : (M → U) → M → M \\
&\operatorname{Sep}␣ P␣ x := \sup␣ \left(∑_{i : T␣\bar x} P␣(\tilde x␣ i)\right)␣ \left(\tilde x ∘ π₀\right)
\end{align}

We must show that for all $x$ and $P$, that for every $z$ we have
$z ∈ \operatorname{Sep}␣ P␣ x ≃ z ∈ x ∧ T␣(P␣z)$.

We have:
\begin{align}
z ∈ \operatorname{Sep}␣ P␣ x
    &≡ ∑_{p : ∑_{i : T \bar x} T␣(P␣(\tilde x␣i))} \tilde x (π₀␣ p) =_M z \\
    &≃ ∑_{i : T␣\bar x} ∑_{q : T␣(P␣(\tilde x␣i))} \tilde x (π₀␣ (i,q)) =_M z \\
    &≡ ∑_{i : T␣\bar x} ∑_{q : T␣(P␣(\tilde x␣i))} \tilde x␣i =_M z \\
    &≡ ∑_{i : T␣\bar x} \left(T␣(P␣(\tilde x␣ i)) ∧ \tilde x␣i =_M z \right)\\
    &≃ ∑_{i : T␣\bar x} \left(\tilde x␣i =_M z ∧ T␣(P␣(\tilde x␣i)\right)) \\
    &≃ ∑_{i : T␣\bar x} \left(\tilde x␣i =_M z ∧ T␣(P␣z)\right) \\
    &≃ \left(∑_{i : T␣\bar x}\tilde x␣i =_M z\right) ∧ T␣(P␣z) \\
    &≡ z ∈ x  ∧ T␣(P␣z)
\end{align}



\end{proof}


\subsection{Union-replacement}

In \cite{aczelrathjen}, the authors introduce the axiom of Union-Replacement.
We use this axiom instead of separate union and replacement axioms as it seems a
more natural construction to use. For multisets it says that if we have a family
of multisets, indexed by a multiset, we can take their multiset union.



\begin{align*}
\mathtt{(UR)}& &∀ a␣ \left( ∀ x ∈ a␣ ∃ b␣ ∀ y␣ \left( y ∈ b ↔ Q(x,y) \right) \right. \\ &&\left.\vphantom{∀a␣(}→ ∃ c␣ ∀ y␣ \left( y ∈ c ↔ ∃ x ∈ a␣ Q(x,y) \right) \right)
\end{align*}

Rendering this in type theory and applying the translation to multisets we get:

\begin{proposition}
\begin{align*}
\mathtt{(M-UR)}& &∏_{a : M} \left(∏_{i : T\bar a} ∑_{b:M}␣ ∏_{y:M} \left( y ∈ b ≃ Q␣(\tilde a␣i)␣y \right) \right)\\ &&  → ∑_{c : M} ∏_{y:M} \left( y ∈ c ≃ ∑_{ i : T\bar a} Q(\tilde a␣ i)␣y \right)
\end{align*}
where $Q : V → V → Set$ is any relation.
\end{proposition}

\begin{proof}

We define
\begin{align}
&\operatorname{UnionRep} : (a : M) → (\bar a → M) → M \\
&\operatorname{UnionRep}␣ a␣ f := \sup␣ \left(∑_{i : T \bar a} \overline{(f␣ i)}\right)␣ \left(λ p.\widetilde {f␣(π₀␣p)}␣ (π₁␣p)\right)
\end{align}

Let us fix $a : M$. Then, from the assumption of \\
$∏_{i : T\bar a} ∑_{b:M}␣ ∏_{y:M} \left( y ∈ b ≃ Q␣(\tilde a␣i)␣y \right)$,
we can extract $f : T\bar a → M$ such that for all $i : T\bar a$ and all $y:M$
we get $y ∈ (f␣i) ≃ Q␣(\tilde a␣i)␣y $. What we then need, is to show that for
every $y:M$ we have
$y ∈ (\operatorname{UnionRep}␣a␣f) ≃ ∑_{ i∈ T\bar a} Q(\tilde a␣ i)␣y $.

We have

\begin{align}
y ∈ (\operatorname{UnionRep}␣a␣f) 
    &≡ ∑_{p : ∑_{i : T\bar a}\overline{f␣i}} \widetilde {f␣(π₀␣p)}␣ (π₁␣p) =_M y \\
    &≃ ∑_{i : T\bar a} ∑_{j : T \overline{f␣ i}} \widetilde {(f␣i)}␣ j =_M y \\
    &≡ ∑_{i : T\bar a} y ∈ (f␣i) \\
    &≃ ∑_{i : T\bar a} Q(\tilde a␣ i)␣y
\end{align}

\end{proof}




\subsection{Singletons}

In set theory, singletons are usually constructed by pairing an element with itself.
For multisets defining singletons from pairs would not work, as the resulting
multiset would contain the element twice, not once. We therefore will prove that
our model has singletons.


If we were to have a singleton axiom in set theory, it would look like:

\begin{align*}
\mathtt{(SING)}& &∀ a␣ ∃ b␣ ∀ z␣\left( z ∈ b ↔ z = a \right)
\end{align*}
Which for our multisets becomes:

\begin{proposition}
\begin{align*}
\mathtt{(M-SING)}& &∏_{a : M}␣∑_{b:M}␣ ∏_{z:M}␣\left( z ∈ b ≃ z =_M a \right)
\end{align*}
\end{proposition}


\begin{proof}
We define
\begin{align*}
&\operatorname{Sing} : M → M \\
&\operatorname{Sing}␣ a := \sup␣ 1␣ \left(λ i.a\right)
\end{align*}

and prove that for every $a,z : M$ we have
$\left(z ∈ \operatorname{Sing}␣ a \right) ≃ \left(z =_M a\right)$.

\begin{align}
z ∈ \operatorname{Sing}␣a &≡ ∑_{i : 1} \left(λ i. a\right)␣i =_M z\\
                          &≡ ∑_{i : 1} a =_M z\\
                          &≡ 1 ∧ (a =_M z)\\
                          &≃ z =_M a
\end{align}
\end{proof}

\emph{Notation:} We will from now on use the notation $\{a\} := \operatorname{Sing}␣a$.



\subsection{Pairing}

The axiom of pairing,
\begin{align*}
\mathtt{(PAIR)}& &∀ a␣ ∀ b␣ ∃ c␣ ∀ z␣\left( z ∈ b ↔ \left(z = a ∨ z = b\right)\right),
\end{align*}
becomes

\begin{proposition}
\begin{align*}
\mathtt{(M-PAIR)}& &∏_{a : M}␣∏_{b:M}␣∑_{c:M}␣ ∏_{z:M}␣\left( z ∈ c ≃ \left( z =_M a ∨ z =_M b\right)\right)
\end{align*}
\end{proposition}


\begin{proof}
First, define

\begin{align}
&p : M → M → 2 → M\\
&p␣ a␣ b␣ (l␣*) := a \\
&p␣ a␣ b␣ (r␣*) := b
\end{align}

Then, let us define
\begin{align*}
&\operatorname{Pair} : M → M → M \\
&\operatorname{Pair}␣ a␣ b:= \sup␣ 2␣ \left(p␣a␣b\right)
\end{align*}

It remains to show that for all $a,b,z ∈ M$ we have
$z ∈ (\operatorname{Pair}␣a␣b) ≃ \left(z =_M a ∨ z =_M b \right)$.

\begin{align}
z ∈ (\operatorname{Pair}␣a␣b) &≡ ∑_{i : 2} p␣i =_M z\\
                                &≃ p␣(l␣*) =_M z ∨  p␣(r␣*) =_M z \\
                                &≡ a =_M z ∨ b =_M z \\
                                &≃ z =_M a ∨ z =_M b
\end{align}
\end{proof}

Notation: We will from now on use the notation $\{a,b\} := \operatorname{Pair}␣a␣b$.



\begin{lemma}
\label{tuple-equality}
For all $a,b,a',b' : M$,
\begin{align}
\{a\} =_M \{a'\} &≃ a =_M a' \\
\{ a,b \} =_M \{ a',b' \} &≃ \left( (a = a' ∧ b=b') ∨ (a = b' ∧ b = a'\right).
\end{align}
\end{lemma}

\paragraph{Example} \label{doubleton} \textbf{The singleton with two elements}

Observe that $(\{∅,∅\} = \{∅,∅\}) ≃ 2$. This leads to the perhaps surprising fact
that

\begin{align}
\left(\{∅,∅\} ∈ \{\{∅,∅\}\}\right) ≃ 2.
\end{align}
This might leave us feeling a bit uneasy, as this is supposed to be a singleton,
not a ``doubleton'', but we will see later (Example
\ref{singleton-example}) how to construct a multiset in which
$\{∅,∅\}$ occurs but once, and that this construction is somewhat like a
quotient of the singleton. For the time being we accept this slight anomaly as a
consequence of our rules.

\paragraph{Remark:} Using singletons, pairs and union we can construct any
finite tupling
of elements of $M$. As we see from the binary case (\ref{tuple-equality}),
the induced mapping $M^n → M$ is not an embedding.


\subsection{Ordered Pairs}

In set theory there are many equivalent ways to encode ordered pairs from
unordered pairs. The most common one, the Kuratowski encoding, defines
$\langle a,b \rangle = \{\{a\},\{a,b\}\}$. It satisfies the characteristic
property, that for all $a,b,a',b'$,

\begin{align}
\langle a,b \rangle = \langle a',b' \rangle ↔ \left(a = a' ∧ b = b'\right)
\end{align}

To understand ordered pairs of multisets, we should therefore require that for all
$a,b,a',b' : M$

\begin{align}
\langle a,b \rangle = \langle a',b' \rangle ≃ \left(a =_M a' ∧ b =_M b'\right)
\end{align}

However, this is not satisfied by mimicking the Kuratowski encoding. We can see
this by letting $a = b = a' = b = ∅$. Given this, we can calculate that
$\{\{a\},\{a,b\}\} =_M \{\{a'\},\{a',b'\}\} ≃ 2$, while \hfill \newline
$\left(a =_M a' ∧ b =_M b'\right) ≃ 1$.

In stead of the Kuratowski encoding, we use the older definition of 
\cite{wiener1914}, $\langle a,b \rangle = \{\{\{a\},∅\},\{\{b\}\}\}$,
which harmonises with the multiset version of the characteristic property.


\begin{proof}
Observe that $\{\{a\},∅\}≠_M\{\{b\}\}$ and $\{a\}≠_M ∅$. So we get that

\begin{align}
\langle a,b \rangle =_M \langle a',b' \rangle 
   &≡ \{\{\{a\},∅\},\{\{b\}\}\} =_M \{\{\{a'\},∅\},\{\{b'\}\}\} \\
   &≃ \{\{a\},∅\} =_M \{\{a'\},∅\} ∧ \{\{b\}\} =_M \{\{b'\}\} \\
   &≃ (\{a\} =_M\{a'\} ∧ ∅ =_M ∅) ∧ (\{b\} =_M \{b'\}) \\
   &≃ a =_M a' ∧ b =_M b'
\end{align}
\end{proof}

\subsection{Cartesian products}

We obtain the cartesian product of two multisets by nesting
$\operatorname{UnionRep}$ around pairing.


\begin{definition}
Given $a,b: M$ define
\begin{align}
a × b := \operatorname{UnionRep}␣ a␣ (λ i.\operatorname{UnionRep}␣ b␣ (λ j. \langle \tilde a␣ i, \tilde b␣ j \rangle) )
\end{align}
\end{definition}
Each pairing can occur multiple times in the cartesian product. To be precise $\langle x,y \rangle ∈ \left(a× b\right) ≃ \left(x ∈ a\right) × \left(y ∈ b\right)$.



\subsection{Functions}
\label{multiset-functions}

There are several choices one could make as to what constitutes a function
between multisets. Just like in set theory, where a function between sets is it
self a set\,—\,namely a set of pairs\,—\,we should like functions between
multisets themselves to be multisets. Therefore, a given pair
$\langle x, y \rangle$ cannot occur an unbounded number of times in a function,
as we then would have problems collecting functions into exponential multisets.

The weakest notion of a function between two multisets is just a map of
occurrences. We will refer to this as a “multiset operation”. Often one consider
the stricter notion which sends equal occurrences to equal occurrences. This
notion we will denote by “multiset function”. As we will now see, we can express
both in our model.

In the model, the notion of a multiset operation between $\sup␣A␣f$ and
$\sup␣B␣g$ corresponds exactly to a map $φ : A → B$, and the stricter notion
adds the requirement that if $f␣a =_M f␣a'$ then $g␣(φ␣a) =_M g␣(φ␣a')$. The
stricter notion corresponds to functions in Aczel’s $V$, but the weaker notion is
equivalent to the stricter notion in the case of $\sup␣A␣f$ and $\sup␣B␣g$ being
sets, in the sense of $A$ and $B$ being of type level $0$ and $f$ and $g$ being
injections. Therefore, we can consider both an extension of the notion of
function to multisets.

The question we will now entertain is: How to capture these two notions in the
kind of formulas we have so far considered for other axioms? Starting with the
operations, we remind our selves that, for iterative sets, a function
$f : A → B$ is a subset of $A×B$, such that the projection down to $A$ is a
bijection. Having equivalences available in our language, we can use the
fibrewise equivalence lemma\footnote{Lemma \ref{fibre-equiv}} to describe the corresponding
situation for multisets.


\begin{definition}
We define the weak notion of a multiset function as follows.
\begin{align*}
\operatorname{Operation} : M →& M → M → Set \\
\operatorname{Operation}_{a␣b}␣f ≔ &\left(∏_z␣z ∈ f → ∑_x␣∑_y␣z=\langle x , y \rangle \right) \\ 
                                ∧ &\left(∏_x␣x ∈ a ≃ ∑_y \langle x , y \rangle ∈ f \right) \\
                                ∧ &\left(∏_y␣y ∈ b ← ∑_x \langle x , y \rangle ∈ f \right) 
\end{align*}
\end{definition}

Observe that weakening the ${≃}$ to ${↔}$ does not give the usual definition of
a function for sets, but rather that of a total binary relation. Total binary
relations form a set in classical set theory, but in CZF this is weakened to the
subset collection axiom which states that there is a set of total relations in
which every total relation has a refinement. We will later prove that the
collection of multiset operations form a multiset, and this should be seen a
form of subset collection / fullness.

\begin{definition}
\label{operation-definition}
We define the notion of a multiset function as follows.
\begin{align*}
&\operatorname{Function} : M → M → M → Set \\
&\operatorname{Function}_{a␣b}␣f ≔ \operatorname{Operation}_{a␣b}␣f ∧ ∏_{x,x',y,y'}␣&&\left(\langle x , y\rangle ∈ f ∧ \langle x' , y' \rangle ∈ f \right) \\ &&& → x = x' → y = y'
\end{align*}
\end{definition}

\subsection{Fullness, subset collection and operations}

In constructive set theory the axiom of fullness states that for each pair of
sets $a$,$b$ there is a set of total relations from $a$ to $b$ such that any
total relation has a restriction to these. The equivalent (relative to the rest
of the axioms of CZF) axiom of subset collection is a variation of fullness
which avoids the complication of using pairs to encode relations.


\begin{align*}
\mathtt{(SUB-COLL)} & &&
∀a,b∃u∀v (∀x∈a∃y∈b Q(x,y) \\
&&& → ∃z∈u (∀x∈a∃y∈z Q(x,y) ∧ ∀y∈z∃x∈a Q(x,y)))
\end{align*}


An unfortunate feature of the subset collection axiom is that it states the
existence of certain sets without defining them uniquely. Classically, the sets
of functions would satisfy the property of fullness. In fact, the requirement
that the set of functions satisfying the fullness property is equivalent to the
axiom of choice. This raises the question of what the constructive nature of this
set really is.

Some insight on the matter can be found by studying Aczel’s model of CZF in type
theory. There the underlying type of the subset collection set between
$\sup␣A␣f$ and $\sup␣B␣g$ is the function type $A → B$. In other words, the
subset collection sets are sets of operations. However, the first order language
of set theory is extensional, and thus unable to exactly pin down what an
operation is, thus the sets of which the axiom claim existence are left
indefinite by the axiom itself. In this respect, the axiom for multisets, in our
language where we have borrowed the connective ${≃}$ from type theory, stating
the existence of multisets of operations is a refinement of collection/fullness
into a definite axiom, namely \emph{exponentiation for operations}.


\subsection{Exponentiation}
\label{multiset-exp}

We define the exponential of two multisets.

\begin{definition}
Let $a , b : M$ be multisets and define

\begin{align*}
 &\operatorname{Exp}␣a␣b : M \\
 &\operatorname{Exp}␣a␣b := \sup␣ (\bar a → \bar b)␣(λf. \sup␣\bar a␣(λi. \langle \tilde a i , \tilde b (f i) \rangle))
\end{align*}
\end{definition}

Next, we formulate the exponentiation axiom for multisets and prove that there exists
a multiset in our model satisfying this axiom.

\begin{proposition}
\begin{align*}
\mathtt{(M-EXP)}& &∏_{a : M}␣∏_{b:M}␣∑_{c:M}␣ ∏_{z:M}␣\left( z ∈ c ≃ \left( \operatorname{Operation}_{a␣b} z\right)\right)
\end{align*}
\end{proposition}

\begin{proof}
Let $c$ be $\operatorname{Exp}␣a␣b$. Thus, we need to prove that for any
given $z : M$, there is an equivalence
$\operatorname{Operation}_{a␣b}␣z ≃ z ∈ \operatorname{Exp}␣a␣b$. We will
give this equivalence in two steps. (A heuristic reason for why we need to
jump through a hoop here is that
$\operatorname{Operation}_{a␣b}␣z$ has three factors while
$z ∈ \operatorname{Exp}␣a␣b$ has two (dependent ones), and we cannot
construct the equivalence factorwise.  We therefore construct a more
finely grained equivalent which maps factorwise to both.)

\textbf{Step 1.} The type $\operatorname{Operation}_{a␣b}␣z$ is equivalent
to the following data:

\begin{itemize}
\item
  $α : \bar a → ∑_{x,y:M} 〈 x , y 〉 ∈ z$
\item
  $β : ∑_{x,y:M} 〈 x , y 〉 ∈ z → \bar b$
\item
  $ε : α ∘ π₀ = \tilde a$, where
  $π₀ : ∑_{x,y:M} 〈 x , y 〉 ∈ z → M$ extracts the $x$ component.
\item
  $δ : β ∘ \tilde b = π₁$, where
  $π₁ : ∑_{x,y:M} 〈 x , y 〉 ∈ z → M$ extracts the $y$ component.
\item
  $π₀∘π₁∘π₁ : ∑_{x,y:M} 〈 x , y 〉 ∈ z → \bar z$, which extracts the
  $z$-index, is an equivalence.
\end{itemize}

This data can be succinctly expressed by the following commutative
diagram:

\begin{align}
\xymatrix{
 \bar a \ar[ddr]_{\tilde a}\ar[rr]^{α}_{≃} & & ∑_{x,y:M}〈x,y〉 ∈ z \ar[ddl]^{π₀}\ar[ddr]_{π₁}\ar[rr]^{β} & & \bar b \ar[ddl]^{\tilde b}\\
 \\
 & M & & M &
}
\end{align}


The type $\operatorname{Operation}_{a␣b}␣z$ is a product of three factors.
The first factor is equivalent to  $π₀∘π₁∘π₁ : ∑_{x,y:M} 〈 x , y 〉 ∈ z → \bar z$ being
an equivalence, since it says that all elements of $z$ are pairs. The second
factor is equivalent to the data $α$ and $ε$ above, by the fibrewise equivalence
lemma (Lemma \ref{fibre-equiv}). Similarly, the third factor is equivalent
to the data $β$ and $δ$. Thus, we conclude that $\operatorname{Operation}_{a␣b}␣z$
is indeed equivalent to the above data.

\textbf{Step 2.} The data given in step 1 is equivalent to 
$z ∈ \operatorname{Exp}␣a␣b$, which is to say that $z$ is
equal to the graph of a map $\bar a → \bar b$.

\begin{align}
\label{pairing-diagram}
\xymatrix{
  ∑_{x,y:M}〈x,y〉 ∈ z\ar[ddr]_{λ(x,y,p) → 〈x,y〉}\ar[rr]^{π₀∘π₁∘π₁} & & \bar z \ar[ddl]^{\tilde z}\\
 \\
 & M &
}
\end{align}

Given the data in step 1, define $f : \bar a → \bar b$ by $f ≔ β ∘ α$.
Since $π₀∘π₁∘π₁ : ∑_{x,y:M} 〈 x , y 〉 ∈ z → \bar z$ is an equivalence,
which makes the diagram (\ref{pairing-diagram}) commute, we derive that


\begin{align}
 z &= \sup␣\bar a␣(λi . 〈π₀␣(α␣i),π₀␣(π₁␣(α␣i))〉)\\
   &= \sup␣\bar a␣(λi . 〈\tilde a␣i,\tilde b ␣(β␣(α␣i))〉) \\
   &= \sup␣\bar a␣(λi . 〈\tilde a␣i,\tilde b ␣(f␣i)〉)
\end{align}

which is precisely that $z$ is the graph of $f$.

In the other direction, assuming that
$z = \sup␣\bar a (λi . 〈\tilde a␣i,\tilde b ␣(f␣i)〉$, we observe
that $π₀∘π₁∘π₁ : ∑_{x,y:M} 〈 x , y 〉 ∈ z → \bar z$ is in fact an equivalence,
and project the equivalence $q : \bar z ≃ \bar a$ from the assumed equality.
We then factor $f$
into $α ≔ (q∘π₀∘π₁∘π₁)^{-1}$ and $β ≔ f∘q∘π₀∘π₁∘π₁$. The fact that the rest of the
equalities of the data hold, follows from the definition of $α$ and $β$
and that diagram (\ref{pairing-diagram}) commutes.

That this construction is an equivalence is (tedious)
routine verification, from which we spare the reader.


In conclusion, combining the above two steps, we have constructed an equivalence 
$\operatorname{Operation}_{a␣b}␣z ≃ z ∈ \operatorname{Exp}␣a␣b$.

\end{proof}




\subsection{Natural numbers}
\label{natural-numbers-multiset}

The natural number axiom is straightforward to translate, and the
construction is exactly the same as in Aczel's model.

Applying the usual abbreviations,
\begin{align*}
S␣y␣z ≡ ∀x \left(x ∈ z ↔ \left(x ∈ y ∨ x = y\right)\right)
\end{align*}
\noindent which codes the relation $z$ is the successor of $y$, and
\begin{align*}
Z␣z ≡ ∀ x\ \neg x∈z\text{,}
\end{align*}
\noindent coding $z$ is zero – the axiom of infinity in set theory can be expressed as:

\begin{align*}
\mathtt{(INF)}& & ∃ u ∀ z \left(z ∈ u ↔ \left(Z␣z ∨ ∃y ∈ u \ S␣y␣z \right) \right)
\end{align*}

For multisets we give similar definitions of $S$ and $Z$, in order to
define an axiom of infinitity.

\begin{align*}
S␣y␣z &≔ ∏_{x:M} \left(x ∈ z ≅ \left(x ∈ y + x = y\right)\right) \\
Z␣z &≔ ∏_{x:M}\neg x∈z
\end{align*}

\begin{proposition}
\begin{align*}
\mathtt{(M-INF)}& & ∑_{u : M} ∏_{z:M} \left(z ∈ u ≅ \left(Z␣z + ∑_{y:M} y ∈ u ∧ S␣y␣z \right) \right)
\end{align*}
\end{proposition}


\begin{proof}
The construction of a natural number object for $M$ is the same
as the construction for Aczel’s $V$. We define a sequence
of multisets $N : ℕ → M$, by

\begin{align*}
&N␣0 ≔ ∅ \\
&N␣(n+1)≔N␣n ∪ \{N␣n\}
\end{align*}

And let our natural number object be $u = \sup ␣ℕ␣N$. It
just remains to observe that $u$ satisfies the condition of $\mathtt{M-INF}$

\begin{align*}
 z ∈ u &≡ ∑_{n:ℕ} N␣n = z \\
      &≅ z = ∅ ∨ ∑_{n:ℕ} N␣(S n) = z\\
      &≅ z = ∅ ∨ ∑_{n:ℕ} (N␣n ∪ \{N␣n\}) = z\\
      &≅ Z␣z ∨ ∑_{n:ℕ} S␣(N␣n)␣z\\
      &≅ Z␣z ∨ ∑_{y:M} y∈m ∧ S␣y␣z
\end{align*}
\end{proof}


==> multisets/homotopy.tex <==
\section{Homotopic aspects of $M$}

The previous section might seem as though not much have changed going
from the sets $V$ to the multisets $M$. In this subsection we will take a look at
what objects might be in $M$ for which, since we work with the identity type on
$M$, higher homotopies come into play. First of all, we observe that $M$ has
the same number of non-trivial levels of homotopy as $U$ has.




\subsection{Homotopy $n$-type}

Recall from the book ``Homotopy Type Theory''\footcite{hottbook} that 
types can be divided into levels, according to how many times one can
iterate the identity type on the type before it becomes trivial, in 
the sense of being contractible. A type is contractible if it has
an element, which every other element is (uniformly) equal to.
This is captured by the following definitions.

\begin{align}
\operatorname{isContractible}(X) ≔ ∑_{x:X}∏_{x':X}x'=x
\end{align}


\begin{align}
 &\mathtt{is-}(-2)\mathtt{-type}\ X = \operatorname{isContractible}(X) \\
 &\mathtt{is-}(n+1)\mathtt{-type}\ X := ∏_{x,y:X} \mathtt{is-}(n)\mathtt{-type}(\Id␣ x␣ y)
\end{align}

\begin{proposition}
$M$ has the same homotopy $n$-type as $U$.
\end{proposition}
\begin{proof}
If $M$ is homotopy $n$-type, then $U$ is also homotopy $n$-type. This follows from the fact that the following map is an embedding.

\begin{align}
&ι : U → M \\
&ι a := (\sup␣a␣(λ a. ∅))
\end{align}

On the other hand if $U$ has homotopy $n$-type, then we show by $W$-induction on 
$M$ that $M$ also has homotopy $n$-type.

Let $x = (\sup␣a␣f)$ and $y = (\sup␣b␣g)$, and consider $\Id␣ x␣ y$. 
By Lemma \ref{w-id} we know that:

\begin{align}
Id␣ x␣ y ≃ ∑_{α : \Id_U␣a␣b} \Id_{Ta → W} f␣(Bα· g)
\end{align}

From W-induction we have the induction hypothesis that the image of \(f\)
has homotopy \(n\)-type, and by Theorem 7.1.8 in the book\footcite{hottbook}.,
we know that this \(Σ\)-type also has homotopy \(n\)-type,



\end{proof}


\subsection{HITs and multisets}

If our universe has Higher Inductive Types (HITs), we can construct multisets
where the index set is a higher groupoid structure. An interesting fact is that
even if $\bar a$ is a higher groupoid, we can still have that $x ∈ a$ is
$1\text{-type}$ for all $x$ .




\begin{example}
\label{singleton-example}
In Example \ref{doubleton} we saw that the singleton
construction unexpectedly gave
singletons where the single element occurred twice, because of its non-trivial
equalities to itself in $M$. A solution to this is to take the connected
compontent of the element in $M$ as the index set of the singleton, instead of
just $1$, along with the inclusion into $M$. However, this requires the connected
component to be $U$-small, which the usual construction does not guarantee.
Adding that assumption, which we conjecture could hold in general (in homotopical
models), since $M$ is
locally $U$-small, we can construct singletons even for elements of $M$ with
non-trivial self-identities.

For any multiset $x : M$, such that there is $t : U$ which represents the
connected component of $x$, i.e. $α:T␣t ≃ ∑_{y:M}∥x=_My∥_{-1}$, we can
define a the singleton $s␣x␣t␣α := \sup␣t (π₀∘α)$. The map $π₀∘α$ is
an embedding, since $∥x=_My∥_{-1}$ is a mere proposition. It follows that
the fibres $y∈s␣x␣t␣α$ are all propositions, and in particular $x ∈ s␣x␣t␣α$
is contractible.

\end{example}



==> multisets/introduction.tex <==
\section{Introduction}

The purpose of this paper is to describe a model of iterative,
transfinite multisets and to discuss a possible axiomatisation of the
model in the context of univalent Martin-Löf style type theory. Before
describing the model, we discuss existing works on multisets and their
relation to the model at hand.

Usage of multisets has a long history, both in mathematics and in
applications. In classical mathematics one models multisets inside set
theory in various ways. Here follows a brief description of three common
ways of representing multisets.

A very general definition, introduced in \cite{Rado1975}, is that a
multiset on a domain set $X$, consists of an assignment
$X → \text{Card}$, which for each element of the domain specifies the
(possibly transfinite) number of occurrences of the element in the
multiset. Often, this notion is restricted to functions $X → \N$,
which represent multisets where each element occurs finitely many times.

One can also view a multiset as a set $A$ with an equivalence relation
$R$ defined on $A$. The idea is that the elements of $A$ are the
occurrences in the multiset, and the relation $R$ specifies which
occurrences are the same. Thus the number of occurrences of $a \in A$ is
the size of the $R$-equivalence class of $a$.


A third way is to consider a multiset as a family of sets. The index set
of the family corresponds to the domain in Rado's multisets, but instead
of assigning a cardinal number, we have a set of occurrences.

These three approaches illuminate different aspects of multisets, and
even though they are formulated quite differently it is relatively easy
to pass back and forth between them. In fact they would be equivalent if
one removes the constraint that the relation in the second formulation
should be reflexive, or restricts the other two to ensure that each
element in the domain occurs at least once.


Rado's formulation reflects that elements in a multiset occurs a specific
number of times. This can be problematic in a constructive context,
where the notion of cardinality is much more nuanced. This is solved if
one takes the family-of-sets definition, which makes perfect sense
constructively, but requires more thought as to what constitutes
equality between multisets. The notion of equality between multisets is
a topic we will come back to later in this paper.

Considering a multiset as a set with equivalence relation, a setoid,
gives an interesting way to talk about the different between identical
elements and equal elements. The identity of elements in the underlying
set $A$ tells us when occurrences are identical, and the relation $R$
tells us which occurrences are equal. Since the underlying theory is set
theory, we can distinguish equal occurrences in a multiset, but not
identical occurrences.


All three notions describe what we in this paper will refer to as
``flat multisets'', as opposed to ``iterative multisets''. In a flat
multiset, the elements are taken from some domain which may not consist
of other multisets. The iterative multisets have elements which are
multisets themselves, and the collection iterative multisets is
generated in a well-founded manner.

\cite{blizard1988} develops an axiomatisation of iterative
multisets with finite occurrences. The theory is a two-sorted, first-order
theory. The two sorts $N$ and $M$, represent the natural numbers and
multisets respectively. The natural numbers are given by the Peano axioms.
Membership is interpreted as a ternary predicate $-\in_{-}-$, where the
intended interpretation of $x \in_n y$ is that $x$ occurs exactly $n$
times in $y$. The axioms for multisets are then chosen so that one can
reconstruct $ZFC$ internally as the multisets where each element occurs
at most once.

In this paper, we will take a different view on elementhood of multisets
compared to Blizard. Instead of a ternary relation, we will
keep the ${\in}$-relation binary and invoke the propositions-as-sets
attitude of Martin-Löf type theory.


In Martin-Löf type theory one does not generally distinguish the notion
of set from the notion of proposition. The notion of a set, as given by
its canonical elements, corresponds exactly to the notion of a
proposition as given by its canonical proofs. This leads us to give the
binary relation ${\in}$ the typing ${\in} : M → M → \set$. Thus, for
given $x,y : M$, we have that $x \in y$ is a set.
\emph{The natural interpretation is that $x \in y$ is the set of 
occurrences of $x$ in $y$}.

Taking the idea of using types to capture the number of occurrences
further, we need a notion of equivalence of type. This is where
Univalent Type Theory enters the picture. Voevodsky’s univalence
axiom expresses\footcite[gives an exposition.]{awodey2013} that an
identity between type is exactly (equivalent to) an equivalence.
For types which are mere sets this means that two mere sets are
identified if there is a bijection between them.



The model of multisets which we present in this paper is derived from a
model of constructive set theory by \cite{aczel1978}. The
multiset model can in fact be seen as a description of what Aczel's
model looks like through the eyes of type theory with the Univalence
Axiom.




==> multisets/model.tex <==
\section{The model}

In the section we recall Aczel's model of constructive set theory, delve into homotopy
type theory and construct a model of multiset theory.


\subsection{Aczel's model}

The idea behind the construction of Aczel's $V$ type in \cite{aczel1978} is
that, given a universe $U : \set$ with decoding type $T : U → \set$, one can
construct a setoid which captures the iteratively generated sets, where each set
has an index of its elements in $U$. An element can be listed more than once in
the index of the set. The equality relation of the setoid removes the
distinction between equal sets with different representations, making sets equal
if they have the same elements.


\begin{definition}
Given a universe $U$, with decoding function $T : U → \set$, let Aczel's $V$ be
the setoid defined as follows.

{\small
\begin{align*}
&V : \set \\
&V := W_{a : U} Ta \\
\\
&=_V : V → V → \set \\
&(\sup\ a\ f) =_V (\sup\ b\ g) := \left(∏_{i : T a} ∑_{j : T b}  (f␣i) =_V (g␣j)\right) ∧ \left( ∏_{j : T b} ∑_{i : T a} (f␣i) =_V (g␣j) \right)
\end{align*}}

\end{definition}


The way to look at a canonical element $x ≡ (\sup\ a\ f) : V$ is that $a$ is a
code for the index of elements in $x$ and $f : T a → V$ picks out the elements
(i.e. sets) contained in $x$.

\paragraph{Remark.} Notice that the relation $=_V$ is $U$-small, if $U$ has
$Σ$-types and $Π$-types. That is, one can prove by W-induction that for each
pair of elements $x,y : V$, there is a code in $U$ for the type $x =_V y$. This
is important, since we want to use equality to construct indices for new sets.


\begin{definition}
Let elementhood in Aczel's V be defined as follows.

\begin{align}
&{∈} : V → V → \set \\
&x ∈ (\sup␣b␣g) = ∑_{i : Tb} x =_V (g␣i)
\end{align}
\end{definition}

\paragraph{Remark.}

Since the relation \(=_V\) is \(U\)-small, it follows that the relation
\({∈}\) is also \(U\)-small.

Aczel goes on to prove that the setoid \((V,=_V)\),
with the relation \({∈}\), is a model of Constructive Zermelo-Fraenkel
set theory (CZF). In this paper, we take a different path, and ask the
question: What is the nature of elements in \(V\), without taking the
quotient of \(=_V\), and instead considering the identity type on \(V\)?

As noted, a set in \(V\) may have the same element listed several times,
but the equality \(=_V\) erases the distinction between representations
that just differ by the number of times they repeat elements. However we
cannot expect the identity type to do the same. Thus, we expect that the
result will be more like multisets, possibly with the obstacle that
order of elements may play a role. As we will see, this obstacle is
overcome by the \emph{univalence axiom}.



\subsection{The identity type on W-types}

The following result is due to Nils Anders Danielsson
\footcite[only available on-line.]{danielsson2012}.
The result characterises the W-type of a type family \(B : A → \set\),
in terms of the identity type of \(A\) and \(B\), up to equivalence. The
lemma does not make use of the Univalence axiom and can be carried out
in plain Martin-Löf type theory.

A technical detail is that the proof as it stands, relies on
\(η\)-reduction. The justification for this is that we take the function
type in the W-type to be the \(Π\)-type of the logical framework, in
which \(η\)-reduction is customary \footcite{mltt}. This is
also how it is implemented in Agda. However one can carry out the proof
without appeal to the \(η\)-reduction, as \(η\)-reduction holds up to
provable equality (See page 62 of \cite{nps-prog}).


\begin{definition}
Given $A : \set$ and $B : A → \set$, and an element $x : W_AB$ we denote by
$\bar x : A$, and $\tilde x : B \bar x → W_AB$ the operations given by
$\overline {(\sup␣ a␣ f)} ≡ a$ and $\widetilde {(\sup␣ a␣ f)} ≡ f$.
\end{definition}



\begin{lemma}
\label{w-id}
For any $A : \set$ and $B : A → \set$, and all $x, y : W_A B$, there is an
equivalence

\begin{align*}
 \Id_{W_A B} ␣x␣ y ≃ ∑_{α : \Id_A ␣ \overline{x}␣\overline{y}} ␣ \Id ␣\widetilde{x}  ␣ (Bα · \widetilde{y})
\end{align*}
\end{lemma}

\subsection{A model of multisets}

We will now present our model of transfinite, iterative multisets, given a
univalent universe $U : \set$ with decoding function $T : U → \set$. It consists
of a type $M$ of multisets, an equality relation $=_M$ and a relation ${∈}$,
which expresses elementhood. The type $M$ is the same $W$-type as Aczel's $V$.
The equality, however, is logically stricter than Aczel's equality, and, as we
will show, equivalent in a strong sense to the identity type of $M$.


\begin{definition}
\label{model-definition}
 We define
\begin{align*}
&M:\set \text{ by }\\
&M:= W_{a : U} Ta 
\end{align*}
and
\begin{align*}
&=_M : M → M → \set \text{ by }\\
&(\sup␣ a␣ f)=_M (\sup␣ b␣ g) := ∑_{α : T a ≃ T b} ∏_{x: Ta} (fx)=_M(g ␣(α␣ x))
\end{align*}
and
\begin{align*}
&{∈} : M → M → \set \text{ by }\\
&x ∈ (\sup b␣ g) := ∑_{i : Tb} x=_M (g␣ i),
\end{align*}
% where ${≃}$ denotes equivalence of types as defined in the homotopy hype theory book\footcite{hottbook}.
\end{definition}

\paragraph{Remark:} Observe that if $U$ has $Π$-types, $Σ$-types and identity
types, then $=_M$ and $∈$ are $U$-small, just like their corresponding relations
in Aczel's $V$.

\subsection{Equality and the identity type}

\begin{theorem}
\label{id-eq-theorem}
(UA)
For each $x,y : M$, we have $(x=_M y) ≃ \left(\Id_M␣ x␣ y \right)$.
\end{theorem}
\begin{proof}
By W-induction. Assume $a,b : U$ and $f : T a → M$ and $g  : T b → M$. Then

\begin{align*}
(\sup a␣ f)=_M (\sup b␣ g) & ≡ ∑_{α : T a ≃ T b} ∏_{x: Ta} (fx) =_M (g (α x)) \\
 \text{Induction hypothesis\ \ \ \ \ \ }&≃ ∑_{α : T a ≃ T b} ∏_{x: Ta} \Id␣ (f␣x)␣ (g (α x))\\
 \text{Definition of ${\sim}$\ \ \ \ \ }&≡ ∑_{α : T a ≃ T b}  f \sim g · α\\
 \text{Extensionality\ \ \ \ \ \ \ }& ≃ ∑_{α : T a ≃ T b}  \Id␣ f␣ (g · α)\\
 \text{Univalence \ \ \ \ \ \ \ \ }& ≃ ∑_{α : a = b} \Id ␣f ␣ (g · Tα)\\
 \text{Lemma \ref{w-id}\ \ \ \ \ \ }& ≃ \Id␣ (\sup a␣ f)␣ (\sup b␣g)
\end{align*}
\end{proof}

The following lemma is important with respect to constructing multisets from
logical formulas, in analogy to the comprehension axiom of set theory. We assume
that our universe has $+$, $Σ$ and $Π$-types, so if we can only prove that the
base relations ${=_M}$ and ${∈}$ also live in the universe, then we can
interpret all bounded first order formulas as families of types in $U$,
indexed by some product of $M$ with it self. Thus we have the following lemma:


\begin{lemma}
$\Id_M$ is essentially $U$-small, in the sense that for every $x,y : M$ there is
an code $ι␣ x␣ y : U$ such that $T(ι␣ x␣ y) ≃ \Id_M␣ x␣ y$.
\end{lemma}

\subsection{Extensionality}
\label{multiset-extensionality-section}

In set theory, the axiom of extensionality expresses that two sets are
considered equal if they have the same elements. More precisely, two sets $x$
and $y$ are equal if for any $z$ we have that $z ∈ x$ iff $z ∈ y$. This
formulation of extensionality fails for multisets, but a very similar
extensionality axiom may be formulated.

\textbf{The principle of extensionality for multisets:} \emph{Two multisets $x$
and $y$ are considered equal if for any $z$, the number of occurrences of $z$ in
$x$ and the number of occurrences of $z$ in $y$ are in bijective correspondence
(in our symbolism: $z ∈ x ≃ z ∈ y$).}


We will now prove a strong version of this principle for our model. The crucial
part of this is summarised in the following lemmas, concerning the fibres of
functions.


\begin{definition}
Given a function $f : A → B$  we define $\fibre{f} : B → \set$
by $\fibre{f␣b} ≔ ∑_{a:A} \Id␣(f␣a)␣b$
\end{definition}

\begin{lemma}
\label{fibre-fun}
Given function extensionality, for any $A,B,C : \set$, and functions $f : A → C$
and $g : B → C$, the following equivalence holds:

\begin{align}
\left(∑_{α : A → B} g ∘ α \sim f \right) ≃
\left(∏_{c : C} \fibre{f␣c} → \fibre{g␣c} \right)
\end{align}

\end{lemma}


\begin{proof}
 We define the maps γ and δ as follows:

\begin{align*}
&γ :\left(∑_{α : A → B} g ∘ α \sim f \right)  → \left(∏_{c : C} \fibre{f␣c} → \fibre{g␣c} \right) \\
&γ␣(α , σ)␣c␣(a , p) ≔ (σ_a , σ_a·p)
\end{align*}

\begin{align*}
&δ : \left(∏_{c : C} \fibre{f␣c} → \fibre{g␣c} \right) → \left(∑_{α : A → B} g ∘ α \sim f \right) \\
&δ␣F ≔ (λa. π₀ (F␣ (f␣ a) (a , \refl_a)) , λa.π₁ (F␣(f␣ a)␣ (a , \refl_a)))
\end{align*}

Unfolding the definitions shows that $δ␣(γ␣(α , σ)) ≡ (α , σ)$ (up to
η-reduction). \Id-induction on the fibres of $f$ shows that $γ␣(δ␣F) \sim F$. Thus,
by function extensionality, we have the desired equivalence.
\end{proof}


\begin{lemma}
\label{fibre-equiv}
Given function extensionality, for any $A,B,C : \set$, and functions $f : A → C$
and $g : B → C$, the following equivalence holds:

\begin{align}
\left(∑_{α : A ≃ B} g ∘ α \sim f \right) ≃
\left(∏_{c : C} \fibre{f␣c} ≃ \fibre{g␣c} \right)
\end{align}

\end{lemma}

\begin{proof}

The proof goes by showing that the equivalence constructed in \ref{fibre-fun}
preserves equivalences. Since being an equivalence is a $(-1)$-type, the
resulting restriction of \ref{fibre-fun} to equivalences is again an
equivalence.

Let γ and δ be as in \ref{fibre-fun}, and denote by γ' and δ' the same
construction, but with $f$ and $g$ having exchanged roles. First step is to show
that for all $α : A → B$ and $σ : g ∘ α \sim f$, if $α$ is an equivalence, then for
every $c : C$ the function $γ␣(α,σ)␣c : \fibre{f␣ c} → \fibre{g␣ c}$ is an
equivalence. Let $F_c≔γ␣(α,σ)␣c$. We construct the inverse
$F_c^{-1} ≔ γ'␣(α^{-1},σ')$,
where $σ' : f ∘ α^{-1} \sim g$ is the proof obtained by reversing
$σα^{-1} : g ∘ α ∘ α^{-1} \sim f ∘ α^{-1}$ and composing with the proof that $g ∘ α
∘ α^{-1} \sim g$. That $F_c^{-1}$ is indeed an inverse of $F_c$ can be verified by
\Id-induction on the fibres of $f$ and $g$ respectively.

We then show that for all $F$ such that $F␣c : \fibre{f␣ c} → \fibre{g␣ c}$ is
an equivalence for all $c : C$, the function $π₀ (δ␣F) : A → B$ is an
equivalence. Let $α ≔ π₀ (δ␣F)$. Its inverse is given by
$α^{-1} ≔ π₀ (δ' (F^{-1})$,
and the fact that it is an inverse of $α$ stems from the fact
that for any $a : A$ and $c : C$ and $h : \Id␣ (f␣a)␣ c$ we have that the
transport of $(a , \refl_{f a}) : \fibre{f␣ (f␣a)}$ along $h$ is $(a , h)$, and
likewise for $g$.


\end{proof}




\begin{theorem}
\label{multiset-extensionality}
(UA)
Given $x,y : M$, the following equivalence holds.

\begin{align}
 \left(x =_M y \right) ≃ ∏_{z : M} \left( z ∈ x ≃ z ∈ y \right)
\end{align}
\end{theorem}

\begin{proof}

From Theorem \ref{id-eq-theorem} we deduce that
$x ∈ (\sup ␣A␣ f) ≃ \fibre{x␣f}$.
This allows us to reformulate the above equivalence to be an
instance of Lemma \ref{fibre-equiv}.

\end{proof}






==> multisets/notation.tex <==
\section{Notation and background}

The following article is set with type theory as its intended metatheory.
Some results depend on the Univalence Axiom, and are marked as such.
Part of the article is formalised in Agda \footcite[in the references
contains a URL to the source code of the formalisation.]{agdalib},
in particular the more technical lemmas leading up to the extensionality
theorem and the extensionality theorem itself. However, this article is
self contained, and even the proofs for which there exists a formalisation
are here presented in usual mathematical writing.

In ways of notation we will mostly use standard type theoretical
notation, but written out as informal constructive mathematics in the
style of the homotopy type theory book\footcite{hottbook},
rather than giving formal derivations. Our notation deviate a bit from
the book in ways mentioned below.
Mostly, these deviations take us close to how type theory is written in
a formal proof system, such as Agda or Coq.


Application of functions and instantiation of dependent types are denoted
by juxtaposition\,—\,e.g. $f␣a$ or $B␣a$\,—\,leaving a small space between the
function or type and their argument.

We use $A : \set$ to denote that $A$ is a type. 

Definitions are signified by $≔$ with the type of the term often listed
on the line above the definition. Definitional equalities are denoted by $≡$.

The equality sign $=$ is used to denote various equivalence relations — each time
identified with a subscript, unless clear from the context. We will use the notation
$\Id$ for the identity type.

We follow the book\footcite{hottbook} in the definition of equivalence of types, $A ≃ B$,
homotopy of functions, $f \sim g$,
and notions such as \emph{contractible}, \emph{mere proposition}, 
\emph{mere set}, and $n$-type.
For the basic properties of these notions we refer the reader to (\cite{hottbook}).

Many proofs involve showing
equivalences of types, which we strive to demonstrate, as far as possible,
using chains of simpler type-algebra equivalences, such as
$\left(∏_{a:A}∑_{b:B␣a} C␣a␣b\right) ≃ \left(∑_{f : ∏_{a:A}B␣a}∏_{a:A}C␣a␣(f␣a)\right)$.

It is is worth noting that we will consider quantifiers, such as ∀,∃,∏ and ∑ to bind
weakly, so that for instance $∏_{x:a} P␣x → Q␣x$ disambiguates to  $∏_{x:a} (P␣x → Q␣x)$
rather than $\left(∏_{x:a} P␣x \right) → Q␣x$. We sometimes will add the parenthesis to
emphasise this.





% \begin{enumerate}
%   \item Transitivity of ${\cong}$.
%   \item Equivalence given by substitution.
%   \item Subsitution using ${\cong}$.
%   \item ``Theorem'' of choice.
%   \item Double $\sum$
% \end{enumerate}


